Learning Internal Representations (COLT 1995)

Probably the most important problem in machine learning is the preliminary biasing of a learner's hypothesis space so that it is small enough to ensure good generalisation from reasonable training sets, yet large enough that it contains a good solution to the problem being learnt. In this paper a mechanism for {\em automatically} learning or biasing the learner's hypothesis space is introduced. It works by first learning an appropriate {\em internal representation} for a learning environment and then using that representation to bias the learner's hypothesis space for the learning of future tasks drawn from the same environment. An internal representation must be learnt by sampling from {\em many similar tasks}, not just a single task as occurs in ordinary machine learning. It is proved that the number of examples $m$ {\em per task} required to ensure good generalisation from a representation learner obeys $m = O(a+b/n)$ where $n$ is the number of tasks being learnt and $a$ and $b$ are constants. If the tasks are learnt independently ({\em i.e.} without a common representation) then $m=O(a+b)$. It is argued that for learning environments such as speech and character recognition $b\gg a$ and hence representation learning in these environments can potentially yield a drastic reduction in the number of examples required per task. It is also proved that if $n = O(b)$ (with $m=O(a+b/n)$) then the representation learnt will be good for learning novel tasks from the same environment, and that the number of examples required to generalise well on a novel task will be reduced to $O(a)$ (as opposed to $O(a+b)$ if no representation is used). It is shown that gradient descent can be used to train neural network representations and experiment results are reported providing strong qualitative support for the theoretical results.

==> abstract <==
Probably the most important problem in machine learning is the
preliminary biasing of a learner's hypothesis space so that it is
small enough to ensure good generalisation from reasonable training
sets, yet large enough that it contains a good solution to the problem
being learnt.  In this paper a mechanism for {\em automatically}
learning or biasing the learner's hypothesis space is introduced.  It
works by first learning an appropriate {\em internal representation}
for a learning environment and then using that representation to bias
the learner's hypothesis space for the learning of future tasks drawn
from the same environment.

An internal representation must be learnt by sampling from {\em many
similar tasks}, not just a single task as occurs in ordinary machine
learning. It is proved that the number of examples $m$ {\em per task}
required to ensure good generalisation from a representation learner
obeys $m = O(a+b/n)$ where $n$ is the number of tasks being learnt and
$a$ and $b$ are constants. If the tasks are learnt independently ({\em
i.e.} without a common representation) then $m=O(a+b)$.  It is argued
that for learning environments such as speech and character
recognition $b\gg a$ and hence representation learning in these
environments can potentially yield a drastic reduction in the number
of examples required per task. It is also proved that if $n = O(b)$
(with $m=O(a+b/n)$) then the representation learnt will be good for
learning novel tasks from the same environment, and that the number of
examples required to generalise well on a novel task will be reduced
to $O(a)$ (as opposed to $O(a+b)$ if no representation is used).

It is shown that gradient descent can be used to train neural network
representations and experiment results are reported providing strong
qualitative support for the theoretical results.

